Trusted Container Extensions for Container-based Confidential Computing

Cloud computing has emerged as a corner stone of today's computing landscape. More and more customers who outsource their infrastructure benefit from the manageability, scalability and cost saving that come with cloud computing. Those benefits get amplified by the trend towards microservices. Instead of renting and maintaining full VMs, customers increasingly leverage container technologies, which come with a much more lightweight resource footprint while also removing the need to emulate complete systems and their devices. However, privacy concerns hamper many customers from moving to the cloud and leveraging its benefits. Furthermore, regulatory requirements prevent the adaption of cloud computing in many industries, such as health care or finance. Standard software isolation mechanisms have been proven to be insufficient if the host system is not fully trusted, e.g., when the cloud infrastructure gets compromised by malicious third-party actors. Consequently, confidential computing is gaining increasing relevance in the cloud computing field. We present Trusted Container Extensions (TCX), a novel container security architecture, which combines the manageability and agility of standard containers with the strong protection guarantees of hardware-enforced Trusted Execution Environments (TEEs) to enable confidential computing for container workloads. TCX provides significant performance advantages compared to existing approaches while protecting container workloads and the data processed by them. Our implementation, based on AMD Secure Encrypted Virtualization (SEV), ensures integrity and confidentiality of data and services during deployment, and allows secure interaction between protected containers as well as to external entities. Our evaluation shows that our implementation induces a low performance overhead of 5.77% on the standard SPEC2017 benchmark suite.

==> sections/discussion.tex <==
%!TEX root = ../main.tex
\section{Discussion}
\label{discussion}
In this section, we discuss possible extensions of \arch. First we discuss approaches to strengthen the security of the underlaying TEE with mechanism against side-channel attacks. Afterwards we describe additional features that can extend \arch.

% \subsection{Support for Currently Available TEEs}
% Supporting a large variety of TEE implementation is a desirable future goal for our novel architecture. There are multiple requirements for a TEE implementation in order to be sufficient. First, we give an insight into existing industry TEE solutions.

% \textbf{ARM TrustZone.} TrustZone introduces two execution worlds in ARM CPUs: The normal world and the secure world. With the introduction of TrustZone, ARM also introduces a new privilege model for their processors. The highest privileged code is called \textit{Secure Monitor}. All other 3 privilege levels for hypervisors, the OS and userland programs exist both in the normal secure world. The main pitfall of TrustZone is the support of only one TEE instance, which leads to hardware vendors only allowing their code to run in the secure world in real-world devices (TODO: references).

% \textbf{Intel SGX.} As SEV, Intel SGX allows the creation of multiple TEE instances at the same time. However, SGX aims to offer enclaves which run in user programs only, and therefore don't have extensive access to the rest of the system as a TrustZone enclave. SGX enclaves can also only be entered or exited through predefined locations and have a limit amount of memory available. Furthermore, SGX allows only to load enclaves which are signed by Intel. This is an additional burden for developers, as it raises the bar for acceptance significantly.

% The only feature which is present in all TEEs is the strong runtime isolation of the secure environment. However, there exist other possible features, which are a requirement for being able to be used for our architecture:

% \begin{itemize}
%     \item Verifiable State: As the secure deployment of the Root VM and Container VMs has be be verifiable, the TEE implementation needs to support attestation. This way, the system, which deploys a VM, can be assured that the VM will be booted in a secure state.
%     \item Secret Injection: Our implementation provides identities to the Root VM and Container VMs via a secure channel. We use secret injection in order to pass an identity to a VM before boot, such that all secure channel establishment with the according VM results in a mutually authenticated channel.
%     \item Multiple TEE Instances: As cloud service providers aim to utilize their hardware at a high capacity, it is favorable to execute many different TEE instances on the same device. Furthermore, the feature of secure channels between secure containers on the same Host System builds upon this requirement.
% \end{itemize}
% \begin{table}[H]
% \centering
% \begin{tabular}{ c | c | c }
% \toprule
%  & Intel SGX & ARM TrustZone \\
%  \midrule
 
% Target & \shortstack{Consumer\&\\Server} & \shortstack{Mobile \&\\Embedded} \\
% Strong isolation & \checkmark & \checkmark \\
% Multiple Enclaves & \checkmark & \cross \\ 
% Attestation & \checkmark & \cross \\ 
% Secret injection & \checkmark & \cross \\
% Performance & low & high \\
% \bottomrule
% \end{tabular}
% \caption{Comparison of TEE Implementations and their Applicability for Remote Secure Containers}
% \label{teecomparison}
% \end{table}
% Table \ref{teecomparison} shows which needed features are supported by SGX and TrustZone. It can be seen that TrustZone does not support all needed features, but SGX does. However, downsides of SGX and related work building upong SGX will be discussed in the next section.

\delete{\subsection{Defenses against Cache Side Channels and Controlled-channel Attacks}
Cache side-channel and controlled-channel attacks are a major threat to confidential computing, especially as existing commercial TEEs do not protect against them. SEV is no exception here. While we consider measures to mitigate these attacks orthogonal to our work, we give an overview over approaches from the literature that aim to mitigate these attacks.

One approach to prevent cache-side-channel attacks is side-channel-resilient algorithms~\cite{primeprobe,constant-time-bernstein}. Yet, a recent attack on time-constant AES implementations highlights that designing and implementing side-channel-resilient algorithms is challenging~\cite{moghimi2019memjam}. Other defense approaches either leverage randomization~\cite{brasser2019dr,newcache} to prevent cache side-channel attacks, or aim to actively detect them in privileged software~\cite{detect_side_channels,perf_counter, timewarp}.
To mitigate controlled-channel attacks, various countermeasures have been proposed recently~\cite{preventing_page_faults,shih2017t-sgx,ahmad2018obliviate,ryoan}. These approaches hide the page-table access patterns from a potentially malicious OS. However, none of them are integrated in commercial TEE architectures and all of them yield a non-negligible performance overhead.}

\delete{\subsection{Possible Extensions}
There are multiple ways how our implementation of \arch can be extended with additional features.

One desirable feature for different use-cases %, such as the use-case evaluated in \Cref{sec:evaluation:performance} where NGINX and MariaDB collaborate, 
is the possibility to have a shared encrypted volume between multiple containers. Our current \arch-implementation does not support Docker Volumes. Volumes are a feature of Docker to mount a host folder in a container, e.g., for persistent data storage. While integrating Docker volumes itself is a pure engineering task, they introduce important security consequences. If data is simply stored in cleartext in the host system, its integrity might be impaired and allows, e.g., rollback attacks. This might lead to problems if container developers are not aware of this fact. For instance, Graphene-SGX~\cite{tsai2017graphene} addresses this with developer-specified positive-lists. Hence, we leave this as an open engineering task for future work.

Another possible extension to our \arch-implementation would be minimizing the overall TCB by building the \vendorvm on a smaller kernel with strong security focus, such as the formally verified seL4~\cite{sel4}, rather than using a standard Linux. However, to the best of our knowledge, Linux is currently the only existing SEV-capable operating system which offers a high flexibility and support for many different devices. Implementing SEV and even SEV-ES or SEV-SNP support in another OS is a time-consuming engineering task which we leave for future work.

The \arch architecture can also be extended to support other cloud-native workloads, like PaaS and SaaS offerings providing Microservices. \arch's isolation, validation and communication mechanisms can be used to protect these workloads in similar ways as containers are protected by \arch.}
